A Systematic Study of Time Limit Exceeded Errors in Online Programming Assignments

Online programming platforms such as Codeforces and LeetCode attract millions of users seeking to learn to program or refine their skills for industry interviews. A major challenge for these users is the Time Limit Exceeded (TLE) error, triggered when a program exceeds the execution time bound. Although designed as a performance safeguard, TLE errors are difficult to resolve: error messages provide no diagnostic insight, platform support is minimal, and existing debugging tools offer little help. As a result, many users abandon their submissions after repeated TLE failures. This paper presents the first large-scale empirical study of TLE errors in online programming. We manually analyzed 1000 Codeforces submissions with TLE errors, classified their root causes, and traced how users attempted to fix them. Our analysis shows that TLE errors often arise not only from inefficient algorithms but also from infinite loops, improper data structure use, and inefficient I/O, challenging the conventional view that TLEs are purely performance issues. Guided by these findings, we introduce Nettle, the first automated repair tool specifically designed for TLE errors, and Nettle-Eval, the first framework for evaluating TLE repairs. Integrating LLMs with targeted automated feedback generated by the compiler and test cases, Nettle produces small, correct code edits that eliminate TLEs while preserving functionality. Evaluated on the same 1000 real-world cases, Nettle achieves a 98.5% fix rate, far exceeding the strongest LLM baseline, and all of its repairs pass both Nettle-Eval and the platform's official checker, confirming the reliability of our framework.

==> sec/temp.tex <==
\section{Understanding TLE Errors}
\label{sec:tle-understanding}

To investigate the underlying causes of Time Limit Exceeded (TLE) errors, we manually analyzed real-world submissions from the Codeforces platform. We sampled multiple problems across different difficulty levels and inspected representative failing programs that triggered TLE or related failures. For each case, we examined the full source code, execution logic, and corresponding repair attempts.

Our analysis reveals six distinct patterns of TLE root causes:

\begin{enumerate}
    
    \item \textbf{Inefficient Algorithm}: Inefficient nested loops or brute-force approaches with time complexity that exceeds problem constraints.
    \item \textbf{Inefficient Handling}: Redundant calls to expensive operations (e.g., \texttt{strlen}, \texttt{memset}) or avoidable overhead in hot loops.
    \item \textbf{Improper I/O}: Format mismatches or type errors that result in incorrect loop bounds or hanging input calls.
    \item \textbf{Infinite Loop}: Control-flow bugs that cause non-terminating loops under corner-case inputs.
    \item \textbf{Memory Access}: Access to out-of-bounds array indices causing undefined behavior or silent corruption. Or unnecessary memory cost.
    \item \textbf{Complexity}: Inefficient nested loops or brute-force approaches.
\end{enumerate}

Below, we elaborate on each pattern with concrete examples and analysis.

\para{(1) Inefficient Algorithm.}
Excessive time complexity frequently appears in brute-force attempts\footnote{\url{https://codeforces.com/contest/584/submission/69503297}}:
\begin{lstlisting}[language=Python]
n, t = map(int, input().split())
while True:
    a = random.randrange(10 ** (n - 1), 10 ** n)
    if a % t == 0:
        print(a)
        break
\end{lstlisting}
To avoid the Time Limit Exceeded (TLE) error, the random algorithm usually includes time calculation. For example, recording the beginning time of execution, and replacing the while-loop condition with whether the current time minus the beginning time is less than the time limitation.

\para{(2) Inefficient Handling.}
Some programs repeatedly recompute or accumulate quantities that could be derived directly\footnote{\url{https://codeforces.com/contest/1/submission/9153531}}:
\begin{lstlisting}[language=Python]
while (n%a!=0):
    n+=1
\end{lstlisting}
$n$,$a$ range from $1$ to $10^9$. The time limit is 1 second. In corner cases, this loop runs up to $O(10^9)$ times. Contestants can replace this time-consuming loop with the effective calculation $n=a * math.ceil(n/a)$;


\para{(3) Improper I/O.}
Improper input parsing often results in type errors or unintended long loops\footnote{\url{https://codeforces.com/contest/1/submission/2096008}}:
\begin{lstlisting}[language=Python]
A=input()
n=float(A[0])
a=float(A[4])
cth=1
while (a*cth<n):
    cth+=1
\end{lstlisting}
$n$, $m$, and $a$ are integers ranging from $1$ to $10^9$. Incorrect parsing may result in an illogical variable value. For example, when $n = 1000000$, $a$ will be assigned to $0$, and the loop statement will always be true.


\para{(4) Infinite Loop.}
A typical endless-loop case results from incorrect logical connectors in loop conditions\footnote{\url{https://codeforces.com/contest/379/submission/129184604}}:
\begin{lstlisting}[language=Python]
a,b=map(int,input().split())
while a>=b:
    if a%b==0:
        a=a//b
\end{lstlisting}
If initial values of a and b do not satisify the $if$ condition, the value of variables will never change, resulting in the while-loop condition always being true.


\para{(5) Memory Access.}
Out-of-bounds writes or reads may produce undefined behavior, sometimes manifesting as silent TLEs. Frequent memory allocation and garbage collection costs\footnote{\url{https://codeforces.com/contest/617/submission/111757810}}:
\begin{lstlisting}[language=python]
x=int(input())
steps = [0, 1, 1, 1, 1, 1]
for i in range(6, x + 1):
  steps.append(min([steps[i-5], steps[i-4], steps[i-3], steps[i-2], steps[i-1]]) + 1)
\end{lstlisting}
Unnecessary list creation incurs allocation and garbage collection costs. Together with the maintain of long list $steps$, memory usage affect usage. 

\para{(6) Complexity.}
The simple simulation or nest loops leads to too many operations\footnote{\url{https://codeforces.com/contest/486/submission/13433966}}:
\begin{lstlisting}[language=python]
n=int(input())
sums=0
for i in range(1,n+1,1):
    sums=sums+((-1)**i)*i
\end{lstlisting}
$n$ ranges from $1$ to $10^{15}$, and the time limitation is 1 second. Too many operations result in the Time Limit Exceeded (TLE) error.


Across these examples, we observe that TLE is a multifaceted failure type encompassing both algorithmic and non-algorithmic issues. Loops may fail to terminate, I/O and type handling may freeze execution, and memory corruption may silently stall the program. Understanding these nuanced causes is crucial for designing feedback systems that go beyond reporting runtime profiling data, enabling targeted and pedagogically meaningful guidance in code repair and learning contexts.
















==> sec/threat.tex <==
\section{Threats to Validity}
\label{sec:threat}

\para{Internal validity.}
One internal threat concerns the possibility that large language models (LLMs) may have memorized some of the Codeforces tasks used in our benchmark. If this were the case, generating correct programs could appear trivial. However, our evaluation centers on repairing existing buggy programs rather than synthesizing new solutions. This repair framing reduces the influence of memorization, as success depends on local edits to flawed code. Moreover, we measure not just correctness but also repair size (edit distance), which emphasizes minimal, targeted changes. We observe that our framework achieves both smaller repairs and higher fix rates with iterative refinement, suggesting active reasoning over rote recall. Additionally, in educational contexts, even if memorization occurs, the primary objective is to provide learners with actionable, interpretable feedback—not to evaluate solution originality.

\para{External validity.}
Our empirical study is based on Codeforces, the largest competitive programming platform. While we believe the TLE cases we analyze are broadly representative of time-bound programming challenges, we do not claim the taxonomy of causes is exhaustive. Our findings may not generalize to domains such as introductory CS courses or early-stage tutorials, where time limits are often absent. However, TLE errors are increasingly common in intermediate and interview-style programming tasks—especially in platforms like LeetCode, HackerRank, and Codility—indicating that our results are relevant to real-world settings where performance constraints matter.\footnote{See, e.g., job-oriented challenges from \url{https://leetcode.com/explore/interview/} and \url{https://www.hackerrank.com/skills-directory}.}

\para{Construct validity.}
A constructive threat involves the alignment between our methodology and the debugging behaviors we aim to model. Our taxonomy of TLE causes and the use of edit distance as a proxy for repair effort are necessarily abstractions. While these constructs offer interpretable and scalable metrics for comparison, they may not fully capture the nuances of human debugging. To mitigate this, we complement our quantitative evaluation with iterative repair experiments, ensuring that the observed trends are robust and not artifacts of a single metric or repair strategy.

